Superconducting properties of tin-copper amorphous thin films

The thermodynamic properties of the superconducting state in the amorphous ${\rm Sn_{1-x}Cu_{x}}$ thin films have been characterized. The concentration of copper changes in the range from $0.08$ to $0.41$. The calculations have been conducted in the framework of the strong-coupling formalism, wherein the Eliashberg functions determined in the tunnel experiment (Phys. Rev. B {\bf 51}, 685 (1995)) have been used. The value of the Coulomb pseudopotential equal to $0.1$ has been adopted. It has been found that the critical temperature ($T_{C}$) decreases from $7$ K to $3.9$ K. The ratio of the energy gap to the critical temperature: $R_{\Delta}=2\Delta\left(0\right)/k_{B}T_{C}$, differs significantly from the BCS value: $R_{\Delta}\in\left<4.4,3.95\right>$. Similarly behaves the ratio of the specific heat jump to the specific heat of the normal state: $R_{C}=\Delta C\left(T_{C}\right)/C^{N}\left(T_{C}\right)$, and the parameter: $R_{H}=T_{C}C^{N}\left(T_{C}\right)/H^{2}_{C}\left(0\right)$, where $H_{C}\left(0\right)$ is the thermodynamic critical field. In particular, $R_{C}\in\left<2.2,1.75\right>$ and $R_{H}\in\left<0.141,0.154\right>$.

==> spis <==
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%[A]
\bibitem{Eisenstein1954A}
J. Eisenstein, Reviews of Modern Physics {\bf 26} (3), 277 (1954).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%[B]
\bibitem{Matthias1963A}
B. T. Matthias, T. H. Geballe, V. B. Compton, Reviews of Modern Physics {\bf 35}, 1 (1963).
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%[1]
\bibitem{Watson1995A}
P. W. Watson, D. G. Naugle, Physical Review B {\bf 51}, 685 (1995).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%[2]
\bibitem{Eliashberg1960A}
G. M. Eliashberg, Soviet Physics-JETP {\bf 11}, 696 (1960).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%[3]
\bibitem{Frohlich1952A}
H. Fr{\"o}hlich, Proceedings of the Royal Society of London A {\bf 215}, 291(1952).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%[4]
\bibitem{Morel1962A}
P. Morel, P. W. Anderson, Physical Review {\bf 125}, 1263 (1962).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%[5]
\bibitem{Ania2013A}
R. Szcz{\c{e}}{\'s}niak, E. A. Drzazga, A. M. Duda, Solid State Communiations {\bf 166}, 50 (2013).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%[6]
\bibitem{Ania2014A}
R. Szcz{\c{e}}{\'s}niak, A. M. Duda, E. A. Drzazga, M. A. Sowi{\'n}ska, Physica C {\bf 506}, 115 (2014).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%[7]
\bibitem{Ania2014B}
R. Szcz{\c{e}}{\'s}niak, A. M. Duda, E. A. Drzazga, Physica C {\bf 501}, 7 (2014).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%[8]
\bibitem{Ania2014C}
E. A. Drzazga, R. Szcz{\c{e}}{\'s}niak, A. M. Duda,  Physica B {\bf 445}, 68 (2014).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%[9]
\bibitem{Ania2014D}
A. P. Durajski, R. Szcz{\c{e}}{\'s}niak, A. M. Duda, Solid State Communiations {\bf 195}, 55 (2014).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%[10]
\bibitem{Ania2015A}
M. W. Jarosik, I. A. Wrona, A. M. Duda, Solid State Communiations {\bf 219}, 1 (2015).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%[11]
\bibitem{Ania2015B}
R. Szcz{\c{e}}{\'s}niak, M. W. Jarosik, A. M. Duda, Advances in Condensed Matter Physics Volume 2015, Artile ID 969564, 10 pages.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%[12]
\bibitem{Marsiglio1988A}
F. Marsiglio, M. Schossmann, J. P. Carbotte, Physical Review B {\bf 37}, 4965 (1988).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%[13]
\bibitem{McMillan1968A}
W. L. McMillan, Physical Review {\bf 167}, 331 (1968). 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%[14]
\bibitem{Allen1975A}
P. B. Allen, R. C. Dynes, Physical Review B {\bf 12}, 905 (1975). 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%[15]
\bibitem{Bardeen1964A}
J. Bardeen, M. Stephen, Physical Review {\bf 136}, A1485 (1964). 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%[16]
\bibitem{Bardeen1957A}
J. Bardeen, L. N. Cooper, J. R. Schrieffer, Physical Review {\bf 106}, 162 (1957).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%[17]
\bibitem{Bardeen1957B}
J. Bardeen, L. N. Cooper, J. R. Schrieffer, Physical Review {\bf 108}, 1175 (1957).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%[18]
\bibitem{Varelogiannis1997A}
G. Varelogiannis, Zeitschrift fur Physik B Condensed Matter {\bf 104}, 411 (1997).

